SPIDER: Fuzzing for Stateful Performance Issues in the ONOS Software-Defined Network Controller

Performance issues in software-defined network (SDN) controllers can have serious impacts on the performance and availability of networks. In this paper, we consider a special class of SDN vulnerabilities called stateful performance issues (SPIs), where a sequence of initial input messages drives the controller into a state such that its performance degrades pathologically when processing subsequent messages. Uncovering SPIs in large complex software such as the widely used ONOS SDN controller is challenging because of the large state space of input sequences and the complex software architecture of inter-dependent network services. We present SPIDER, a practical fuzzing framework for identifying SPIs in this setting. The key contribution in our work is to leverage the event-driven modular software architecture of the SDN controller to (a) separately target each network service for SPIs and (b) use static analysis to identify all services whose event handlers can affect the state of the target service directly or indirectly. SPIDER implements this novel dependency-aware modular performance fuzzing approach for 157 network services in ONOS and successfully identifies 10 new performance issues. We present an evaluation of SPIDER against prior work, a sensitivity analysis of design decisions, and case studies of two uncovered SPIs.

==> figs/__latexindent_temp.tex <==
\Input{the analyzed service $\fservice$, the dependencies $\fcontext$}
\Output{a list of events $\feventlist$}
$\fgenerator_{\feventtypelist_\fservicelist}\leftarrow 
\mathrm{EventListGenerator}(\feventtypelist)$\;
$\ftime_{max}\leftarrow 0$\;
$\feventlist\leftarrow \emptyset$\;
$\finputlist\leftarrow \mathrm{\random}\cdot\emptyset$\;
\While {$\mathrm{shouldContinue}()$} {
  \For {$\finput\in\finputlist$} {
    $\mathrm{InitServices}(\fservicelist)$\;
    $\finput'\leftarrow\mathrm{\fmutate}(\finput)$\;
    $\langle\fstate_\fservicelist,events\rangle\leftarrow 
    \mathrm{\fgenerator_{\fstatetypelist_\fservicelist}}(\finput', 
    \fgenerator_{\feventtypelist_\fservicelist})$\;
    $\fevent\leftarrow 
    \mathrm{\fgenerator_{\feventtypelist_\fservicelist}}(\finput')$\;
    $\fdata\leftarrow\mathrm{execute}(\fservicelist, \fstate_\fservicelist, \fevent)$\;
    \If {$\mathrm{\fguidance}(\fdata)$}{
      $\finputlist\leftarrow \finputlist\cdot \finput'$\;
    }
    \If {$\fdata_{\ftime}> \ftime_{max}$}{
      $\ftime_{max}\leftarrow \fdata_{\ftime}$\;
      $\feventlist\leftarrow events\circ\fevent$\;
    }
  }
}
\Return{$\feventlist$}


==> figs/decomposing.tex <==

\pgfplotstableread[row sep=\\,col sep=&]{
        interval & carT & carR \\
        CastorArpManager & 2 & 47 \\
        DeviceManager & 5 & 46 \\
        BgpRouter & 2 & 46 \\
        DhcpManager & 12 & 47 \\
        DhcpRelayManager & 7 & 46 \\
        HostManager & 3 & 46 \\
        IntentMonitorAndRerouteManager & 3 & 3 \\
        HostMobility & 8 & 46 \\
        MyTunnelApp & 11 & 46 \\
        PortStatisticsManager & 3 & 46 \\
        VbngManager & 7 & 50 \\
        VirtualPublicHosts & 1 & 46 \\
        VplsManager & 3 & 47 \\
        HostToHostIntentCompiler & 4 & 46 \\
        }\erctwenty

\begin{tikzpicture}
\begin{axis}[
        ybar,
        bar width=.15cm,
        width=\textwidth,
        height=.35\textwidth,
        % x tick label style  = {text width=1cm,rotate=30},
        x tick label style={rotate=30, anchor=east, align=center},
        legend style={at={(0.5,1.0)},
            anchor=north,legend columns=-1},
        symbolic x coords={CastorArpManager,DeviceManager,BgpRouter,DhcpManager,DhcpRelayManager,HostManager,IntentMonitorAndRerouteManager,HostMobility,MyTunnelApp,PortStatisticsManager,VbngManager,VirtualPublicHosts,VplsManager,HostToHostIntentCompiler},
        xticklabels={arp,device,bgp-router,dhcp,dhcp-relay,host,imr,mobility,p4-tutorial,port-statistics,vbng,vph,vpls,h2h-intent},
        xtick=data,
        %nodes near coords,
        %nodes near coords align={vertical},
        % ymin=0,ymax=100,
        ylabel={\# of services in each group},
    ]
    \addplot table[x=interval,y=carT]{\erctwenty};
    %\addplot table[x=interval,y=carD]{\erctwenty};
    \addplot table[x=interval,y=carR]{\erctwenty};
    \legend{{\systemname}, W/O Pruning}
\end{axis}
\end{tikzpicture}

==> figs/drivers.tex <==
\Input{The type of the state $\ftype$, random number
  generator provided by the fuzzer $\frandom$}
\Output{An instance $\fstate$ of the type $\ftype$}
\SetKw{Continue}{continue}
\SetKwFunction{Fn}{Instantiate}{:}{}
\SetKwProg{FInstantiate}{Instantiate}{:}{}
\FInstantiate{$\ftype, \frandom$} 
{
  \If {$\ftype=\mathrm{Int}$} {
    $\fstate\leftarrow\mathrm{randomInt}(\frandom)$\;
  }
  \If {$\ftype=\mathrm{List}\ \ftype'$} {
    $\fstate\leftarrow \emptyset$\;
    \For{$0<i<\mathrm{LIST\_SIZE}$}{
      $L\leftarrow L\circ \Fn{$\ftype',\frandom$}$
    }
  }
  \If {$\ftype=\mathrm{Record}\ \{\flabel_i: \ftype_i^{i\in 1..n}\}$} {
    $\fstate\leftarrow \fstate[ l_i\mapsto \Fn{$\ftype_i,\frandom$} | i\in 1..n ]$\;
  }
  \Return{$\fstate$}
}


\SetKwProg{FEither}{Either}{:}{}

\FEither{$\ftype_1, \ftype_2, \frandom$}{
  \If{$\mathrm{randomBoolean}(\frandom)$}{
    \Return{$(\Fn{$\ftype_1, \frandom$}, nil)$}\;
  }
  \Else {
    \Return{$(nil, \Fn{$\ftype_2, \frandom$})$}\;
  }
}

\SetKwProg{FOptional}{Optional}{:}{}
\FOptional{$\ftype, \frandom$}{
  \If{$\mathrm{randomBoolean}(\frandom)$}{
    \Return{$\Fn{$\ftype, \frandom$}$}\;
  }
  \Else {
    \Return{$nil$}\;
  }
}

\SetKwProg{FAtLeastOne}{AtLeastOne}{:}{}
\FAtLeastOne{$\ftype_1, \ftype_2, \frandom$}{
  $\fstate_1, \fstate_2\leftarrow nil$\;
  \If{$\mathrm{randomBoolean}(\frandom)$}{
    {$\fstate_1\leftarrow\Fn{$\ftype_1, \frandom$}, nil$}\;
  }
  \If {$\fstate_1=nil\lor\mathrm{randomBoolean}(\frandom)$}{
    {$\fstate_1\leftarrow\Fn{$\ftype_1, \frandom$}, nil$}\;
  }
}


==> figs/fuzzing.tex <==
\Input{the analyzed service $\fservice$, the dependencies $\fdependency$ 
of the analyzed service}
\Output{a list of events $\feventlist$}
% $\fgenerator_{\feventtypelist_\fservicelist}\leftarrow 
% \mathrm{EventListGenerator}(\feventtypelist)$\;
$\ftime_{max}\leftarrow 0$\;
$\feventlist\leftarrow \emptyset$\;
$\finputlist\leftarrow \mathrm{\random}\circ\emptyset$\;
\While {$\mathrm{shouldContinue}()$} {
  \For {$\finput\in\finputlist$} {
    $\mathrm{InitServices}(\fservice\circ\fdependency)$\;
    $\finput'\leftarrow\mathrm{\mutate}(\finput)$\;
    $events\leftarrow\fgenerator(\finput')$\;
    $\mathrm{Process}(events_{0:-1}, \fservice\circ\fdependency)$\;
    $\feedback\leftarrow\mathrm{Process}(events_{-1}, \fservice)$\;
    \If {$\mathrm{\guidance}(\feedback)$}{
      $\finputlist\leftarrow \finputlist\cdot \finput'$\;
    }
    \If {$\feedback_{\ftime}> \ftime_{max}$}{
      $\ftime_{max}\leftarrow \feedback_{\ftime}$\;
      $\feventlist\leftarrow events$\;
    }
  }
}
\Return{$\feventlist$}


==> figs/main-algo.tex <==
\Input{an SDN controller $\fcontroller$}
\Output{A list of OpenFlow messages $\foflist$}

% $\fstateglobal' \leftarrow \mathrm{\fsystemdatastructure}
% (\fservice, \fstateglobal)$\;
% $\fstateglobal' \leftarrow \{\flabel: \fstateglobal.l\ |\ \flabel\in \flabellist \}$\;

\For{$\fservice\in \fcontroller$} {
$\langle\feventtypelist, \fservicelist\rangle\leftarrow \mathrm{\fsystemslicing}(s, C)$\;
$\feventlist \leftarrow 
\mathrm{\fsystemgenerator}(\feventtypelist, \fservicelist)$\;
\If {$\mathrm{execTime}(\feventlist,\fservicelist)>\fthresholdcpu$} {
$\foflist \leftarrow \mathrm{\fsystemmapping}(\feventlist, \fcontroller)$\;
\Return{$\foflist$}\;
}
}

==> figs/naive-algo.tex <==
\Input{SDN controller $\fcontroller$}
\Output{A list of OpenFlow messages $\fofin$}

$\ffeedback\leftarrow Null$\;
\For{$0 < N < \fthresholdcounter$}{
  \Repeat{timeout}{
    $\fofin \leftarrow \emptyset$\;
    $\mathrm{Init}(\fcontroller)$\; \label{algo:native:init}
    \While{$\mathrm{len}(\fofin) < N$}{
      $\fof \leftarrow \mathrm{GenPacket}(\ffeedback)$\; \label{algo:native:random}
      $\fofin \leftarrow \fofin\circ \fof$\;
      $\ffeedback' \leftarrow \mathrm{Send}(\fcontroller, \fof)$\; \label{algo:native:send}
      \If{$\mathrm{CPUUsage}(\ffeedback') > \fthresholdcpu$}{
        \Return{$\fofin$}\;
      }
      $\ffeedback \leftarrow \mathrm{Merge}(\ffeedback)$
    }
  }
}


==> figs/predicate.tex <==
\begin{alignat*}{1}
  &\mathrm{OneToOne}(\fdatastructure: \mathrm{Map}\ T):
  \forall i,j\in \fdatastructure\ i\not=j\rightarrow
  \fdatastructure\llbracket i \rrbracket \not= \fdatastructure\llbracket j\rrbracket \\
  % &\mathrm{OneEdgeLeaving}(\fdatastructure: \mathrm{Graph}):\\
  % &\quad \forall v\in\fdatastructure.\mathrm{vertices}\ \exists e\in \fdatastructure
  % .\mathrm{edges}\  e.\mathrm{src}=v \land \\
  % &\quad \forall v \in \fdatastructure.\mathrm{vertices}\ e_1, e_2 \in 
  % \fdatastructure.\mathrm{edges}\\
  % &\quad\quad((e_1.\mathrm{src}=v\land e_2.\mathrm{src}=v)
  % \rightarrow e_1=e_2)
  % \\
  &\mathrm{ContainsKey}(i: \mathrm{Int})(\fdatastructure: \mathrm{Map}\ T): i\in \fdatastructure\\
  &\mathrm{Contains}(v: T)(\fdatastructure: \mathrm{List}\ T): v\in \fdatastructure\\
  &\mathrm{Contains}(v: T)(\fdatastructure: \mathrm{Set}\ T): v\in \fdatastructure\\
  &\mathrm{Contains}(v: T)(\fdatastructure: \mathrm{Map}\ T): 
  \exists i\in \fdatastructure\ \fdatastructure\llbracket i\rrbracket = v
\end{alignat*}

==> figs/sdn-controller.tex <==
\Input{A list of SDN services $K$}
\SetKw{Continue}{continue}

$\feventlist \leftarrow \emptyset$\;
$\fdatastructurelist\leftarrow\mathrm{InitDataStructure}()$\;
\While{True} {
  $\fofin \leftarrow \mathrm{receive()}$\;
  \For {$\fof \in \fofin$} {
    $\feventlist \leftarrow \feventlist\circ \mathrm{create\_event}(\fof)$\;
  }
  \If {$\feventlist=\emptyset$} {\Continue\;}
  $\fevent\leftarrow \mathrm{pop}(\feventlist)$\;
  \For {$\fservice \in \fservicelist$} {
    $\factionlist \leftarrow \mathrm{process}(\fservice, \fevent, \fdatastructurelist)$\;
    \For {$\faction \in \factionlist$}{
      \Switch{$\faction$}{
        \Case{$\factionmessage$}{
          $\mathrm{emit}(\factionmessage)$
        }
        \Case{$\factiondatastructure$}{
          $\fdatastructurelist, \feventdatastructure\leftarrow\mathrm{update}(\fdatastructurelist, \factiondatastructure)$\;
          $\feventlist\leftarrow\feventlist\circ\feventdatastructure$
        }
      }
    }
  }
}

==> figs/slicing.tex <==
\Input{The source code of the SDN controller $\fcontroller$, 
a service $\fservice$.}
\Output{The dependencies $\fdependency$ of the input service}
$\fdependency\leftarrow\emptyset$\;
$candidates\leftarrow \{\fservice\}$\;
$\fcallgraph\leftarrow\mathrm{buildCallGraph}(\fcontroller)$\;
\While{$candidates\not=\emptyset$} {
$service\leftarrow\mathrm{pop}(candidates)$\;
\If{$service\in\fdependency$} {
\Continue
}
$\fdependency\leftarrow \fdependency\cup\{service\}$\;
\For {$\langle \ffunction_1, \ffunction_2 \rangle\in \fedge_{\fcallgraph}$} {
    $\fservice_1\leftarrow \mathrm{getService}(\ffunction_1)$\;
    $\fservice_2\leftarrow \mathrm{getService}(\ffunction_2)$\;
    \If{$\ffunction_2\in \ffunctionreadwrite_{service}$} {
        $candidates\leftarrow candidates\circ \fservice_1$\;
    }
    \If{$\fservice_1=service$} {
        $candidates\leftarrow candidates\circ \fservice_2$\;
    }
}
}
% $\feventtypelist\leftarrow \feventtypelist\circ \mathrm{getEvents}(service)$\;
% \For {$function\in service$} {
% \If {$\mathrm{isConstantFunction}(function)$} {
% \Continue
% }
% \For {$caller\in \mathrm{getCallers}(CG, function)$} {
% \If{$\mathrm{isService}(caller)$}{
% $candidates\leftarrow candidates\circ caller$\;
% }
% }
% \For {$callee\in \mathrm{getCallees}(CG, function)$} {
% \If{$\mathrm{isService}(callee)$}{
% $candidates\leftarrow candidates\circ callee$\;
% }
% }
% }
% }
\Return{$\fdependency$}


==> figs/state-generator.tex <==
\Input{An input bit stream $\finput$ from underlying fuzzer and a event 
generator $\fgenerator_{\feventtypelist_\fservicelist}$.}
\Output{A state $\fstate$.}
$\fstate\leftarrow \mathrm{InitState}()$\;
$events\leftarrow \fgenerator_{\feventtypelist_\fservicelist}(\finput)$\;
\For{$\fevent\in events$}{
	$\langle \fstate, \fevent'\rangle\leftarrow\ffunction^\feventlist_\fservice(\fstate, \fevent)$\;
}
\Return{$\langle\fstate, events\rangle$}

==> figs/syn-result.tex <==
\begin{center}
    \begin{tabular}{ l | l | c | c }
     Service & Pattern & {\systemname} & Naive \\ 
     \hline
     HostService&  Linear & \cmark & \xmark \\  
     \hline
     HostService&  Burst & \cmark & \xmark \\  
     \hline
     HostService&  Phase & \multicolumn{2}{|c}{not applicable} \\  
     \hline
     BgpRouter &  Linear & \cmark & \xmark \\  
     \hline
     BgpRouter &  Burst & \cmark & \xmark \\  
     \hline
     BgpRouter&  Phase & \multicolumn{2}{|c}{not applicable} \\  
     \hline
     AclService &  Linear & \cmark & \xmark \\  
     \hline
     AclService &  Burst & \cmark & \xmark \\  
     \hline
     AclService&  Phase & \multicolumn{2}{|c}{not applicable} \\  
     \hline
     DeviceService &  Linear & \cmark & \xmark \\  
     \hline
     DeviceService &  Burst & \cmark & \xmark \\  
     \hline
     DeviceService &  Phase & \cmark & \xmark \\  
     \hline
     DhcpService &  Linear & \cmark & \cmark \\  
     \hline
     DhcpService &  Burst & \cmark & \cmark \\  
     \hline
     DhcpService &  Phase & \cmark & \xmark \\  
     \hline
     DhcpRelayService &  Linear & \cmark & \cmark \\  
     \hline
     DhcpRelayService &  Burst & \cmark & \cmark \\  
     \hline
     DhcpRelayService &  Phase & \cmark & \xmark \\  
     \hline
     IMRService &  Linear & \cmark & \xmark \\  
     \hline
     IMRService &  Burst & \cmark & \xmark \\  
     \hline
     IMRService &  Phase & \cmark & \xmark \\  
    \end{tabular}
\end{center}

==> figs/synthesizing.tex <==
% \Input{A list of network events $\feventlist$ and 
% the SDN controller $\fcontroller$}
% \Output{A list of OpenFlo packets $\foflist$}
% $\foflist\leftarrow\emptyset$\;
% \For{$\fevent\in\feventlist$} {
%     $message\leftarrow\mathrm{CreateSymMessage}()$\;
%     $\langle events, constraints\rangle\leftarrow\mathrm{SymExec}(C, message)$\;
%     \For{$event\in events$} {
%         \If {$\mathrm{sameType}(event, \fevent)$} {
%             $constraints' = constraints \land(event = \fevent)$\;
%             \If{$\mathrm{sat}(constraints')$} {
%                 $\fof\leftarrow\mathrm{solve}(constraints', message)$\;
%                 $\foflist\leftarrow \foflist \circ\fof$\;
%                 \Continue
%             }
%         }
%     }
% }
% \Return{\foflist}

==> figs/transform.tex <==
\begin{mathpar}
  \inferrule{
    c \in \mathrm{Int}
  }{
    \mathrm{readInt}()
  }\and
  \inferrule{
    t \in \mathrm{Var}
  }{
    t
  }\and
  \inferrule{
    e_1\; \mathbf{op}\; e_2
  }{
    \mathrm{transform}(e_1) \;\mathbf{op}\;  \mathrm{transform}(e_2)
  }\and
  \inferrule{
    t = e
  }{
    \mathrm{transform}(t) = \mathrm{transform}(e)
  }\and
  \inferrule{
    s_1s_2
  }{
    \mathrm{transform}(s_1)\mathrm{transform}(s_2)
  }\and
  \inferrule{
    \mathrm{if}\; e\; s
  }{
    \mathrm{if}\;\mathrm{transform}(e)\;\mathrm{transform}(s)
  }\and
  \inferrule{
    \mathrm{while}\; e\; s
  }{
    \mathrm{while}\;\mathrm{transform}(e)\;\mathrm{transform}(s)
  }\and
\end{mathpar}

==> figs/types.tex <==
\begin{alignat*}{1}
  \ftype ::               & = \mathrm{Int}                                                       \\
                     & \quad\, \mathrm{List}\ \ftype                                             \\
                     & \quad\, \mathrm{Set}\ \ftype                                              \\
                     & \quad\, \mathrm{Map}\ \ftype                                              \\
                     & \quad\, \mathrm{Record}\ \{{\flabel}_i: {\ftype}_i^{i\in 1..n}\} 
\end{alignat*}

==> files/__latexindent_temp.tex <==
  \begin{minipage}{0.48\textwidth}
  \inputminted{Java}{./code-samples/HostStore.java}
  \caption{HostStore used by host service.}
  \label{fig:host-store}
  \end{minipage}
\end{figure*}

==> files/conclusions.tex <==
%\section{Conclusions}

%\textbf{}


 %\vyas{if space crunch move this philosophy para to to conclusions} 



%\vyas{one meta thing for the paper management --  id try to write down a prioritized list of concerns/todos from here to deadline so we dont lose track of critical issues. to me the biggest gaping holes are the "fairness" of comparison to blackbox, "toyness" of eval,  "acking lack of completeness" of analysis, "detailed design" writing story. second order issue is consistency of story/terminlogy through the paper}



==> files/event-fuzzer.tex <==
\section{Event-Driven Performance Fuzzing}\label{sec:performance-fuzzer}

\vyas{for this section, we need to expand more on 5.1 and downplay the earlier parts?} 


In order to explore the state space of each service, the fuzzer 
needs to model and mutate each state easily. Most fuzzers generate 
binary input which can be mutated by the fuzzers easily. However, 
binary input is not recognized by services. Semantic fuzzing allows 
developers to implement input generators that map the binary input 
returned by the fuzzer to structured inputs~\cite{zest}. 
This mapping guarantees that every untyped binary input corresponds 
to a valid data structure and bit-level mutation performed by 
performance fuzzer corresponds to structural mutation in the 
data structure. 
The quality of the input generators affects the 
performance of the fuzzer directly.
% Given an input service and a the context set of the service, {\systemname}
% then explores the state space of the input services 
% to find a state that may cause performance issue of the input service.
% However, underlying stateful generator 
% This seems like a promising starting point but implementing 
% state generators is still challenging.
% \vyas{feel like some of this discussion/tradeoff on cost/effort needs to be in sec 3?}

% Event-driven performance fuzzer takes a set of services as input and  
% finds a concrete state of the input service which may have performance 
% vulnerabilities. The intuition is to test the performance 
% of the input services under different states generated by the 
% performance fuzzer. The performance fuzzer needs to satisfy two 
% properties. 1) the fuzzer can generate all possible state of the 
% input services. 2) the fuzzer does not generate any invalid state 
% of the input services.


\paragraph{Constraints in data structures:}
One challenge of implementing state generators is that 
there are constraints and invariants of states in the SDN controller. 
Such constraints and invariants are maintained by each service implicitly.
For example, \texttt{HostStore} shown in Figure~\ref{fig:host-store} maintains 
three invariants: 1) the host stored in \texttt{hosts} map should 
have corresponding \texttt{HostId}; 2) the host stored in 
\texttt{hostsByIp} should have corresponding \texttt{IpAddress};
3) all hosts stored in \texttt{hosts} are also stored in 
\texttt{hostsByIp}. Such invariants are enforced by 
the implementation of the \texttt{HostService}.
% and each time function 
% \texttt{addHost} or function \texttt{updateHost} is
% called, the function makes sure that those 
% invariants are not violated.
% Different data structures implemented in the SDN 
% controller maintains 


% \subsection{State Generation}
% The quality of the state generator affects the fuzzing 
% results directly. 
Violations of any constraints or invariants will cause 
false positives.
% Invalid states, which is not reachable in the SDN controller,
% generated by the generator will cause false positives. 
For example, a \texttt{HostStore} generator may
generate a \texttt{hosts} map which contains the same host 
indexed by different host IDs. Such invalid states are 
harmful not only that they will cause false positives, 
but also that generating and executing an invalid state 
waste the fuzzing resources.
% If the state generator generates 
% invalid states, the fuzzer may report false negatives.
% On the other hand, if a state generator fails to 
% generate certain valid states, the performance fuzzer 
% may miss real vulnerabilities.
% If the state generator fails to explore the entire 
% state space of the SDN controller, the fuzzer 
% may miss real vulnerabilities. 
% However, modelling 
% the state space of the SDN controller is not trivial.
% The quality of generated states affects the fuzzing results 
% directly. If the fuzzer only explores the state space 
% partially, it may miss real vulnerabilities. If the fuzzer 
% generates invalid states, it may report false positives.

Moreover, if a state generator only generates a subset 
of valid states, the fuzzer may miss true positives.
For example, if a \texttt{HostStore} generator only 
generates a \texttt{hosts} map with size smaller than 
five, a fuzzer may never be able 
to identify vulnerabilities that can only be exploited 
when the size of \texttt{hosts} map is larger than 10.
Therefore, an ideal state generator needs to satisfy 
two properties: 1) given a valid state, there is a 
binary input so that the generator will take the binary 
input and return the valid state (completeness); 
2) given a binary input, the state generator will 
generate a valid state (soundness).
% If a \texttt{HostStore}
% generates hosts indexed by wrong host ID, the performance 
% fuzzer may report false warnings.
% the performance fuzzer needs 
% to generate both \texttt{hosts} and \texttt{hostsByIp} 
% correctly. 


\paragraph{Implementation effort:}
In an ideal scenario, we can implement generators for 
each data structure implemented in the SDN controller.
However, implementing generators is both time consuming 
and error-prone. For example, there are more than 500 
different data structures used in the ONOS SDN controller.
Generators cannot be shared between different data structures 
because of different constraints and invariants. Every time 
a new services is introduced, new generators needs to be 
implemented.

% such generators is both time consuming and 
% error-prone. There are more than 500 different 
% data structures implemented in the SDN controller and each 
% data structure contains constraints and invariants. 
% Generators cannot be shared among services and the fuzzer 
% always requires new generators to analyze new services.
% % Every time a new service is introduced, the fuzzer 
% % requires new generators to test the new service.
% Another solution is to implement a universal 
% generator which is able to generate data structures 
% regardless their types. Though a universal 
% state generator requires low implementation effort and 
% does not require modification when a new service is 
% introduced. The universal state
% generators may fail to satisfy the constraints and 
% produce invalid states.
% For example, HotFuzz~\cite{hotfuzz} generates 
% program inputs based on the type of each input.
% However, the constraints such as the relationship 
% between the keys and values stored in a map data 
% structure is not represented in their types.
% If we adopt this design to generate \texttt{HostStore}, 
% the generator may generate hosts indexed by wrong 
% host ID.

% The quality of the state generated by the fuzzer 
% influences the fuzzing performance directly. If the fuzzer 
% only generates a subset states, it may miss real bugs.
% If the fuzzer generates invalid states, it may report 
% false positives. One naive implementation of state generator


% The state of the SDN controller is represented by a tuple of 
% data structures $\fstate=\langle\fdatastructure_1, \fdatastructure_2, 
% \dots, \fdatastructure_N\rangle$ and the type of the state of the SDN controller 
% is represented by a tuple of types of data structures 
% $\fstatetypelist=\langle \fstatetype_1, \fstatetype_2, 
% \dots, \fstatetype_N \rangle$.
% And each service $\fservice$ accesses to a subset of states with type 
% $\fstatetypelist_\fservice=\langle \fstatetype_{i_1}, 
% \fstatetype_{i_2},\dots,\fstatetype_{i_m}\rangle$ where $m<n\land 
% i_j < i_k \text{ iff } j \leq k\land 1 \leq i_1 \land i_m \leq N $.
% Similarly, $\feventtypelist=\langle \feventtype_1, \feventtype_2,\dots,
% \feventtype_N\rangle$  represents all possible types of events that 
% can be generated in the SDN controller and 
% $\feventtypelist_\fservice=\langle \feventtype_{i_1}, 
% \feventtype_{i_2},\dots,\feventtype_{i_m}\rangle$ represents all 
% types of events listened by service $\fservice$. A state $\fstate$ is 
% accepted by service $\fservice$ if the state contains all declared 
% states in $\fstatetypelist_\fservice$ written as 
% $\fstatetypelist_\fservice\models\fstate$. An event $\fevent$ is listened 
% by a service $\fservice$ if the event has one of type declared in 
% $\feventtypelist_\fservice$ written as 
% $\feventtypelist_\fservice\models\fevent$.
 
% A state generator takes a bitstream as input and returns a concrete state 
% and an event, $\fgenerator::\textrm{\fbitstream}\rightarrow\langle 
% \fstate, \fevent\rangle$. A generator can be used to analyze service 
% $\fservice$ if all states and events generated by the generator 
% satisfy that $\fstatetypelist_\fservice\models\fstate\land
% \feventtypelist_\fservice\models\fevent$.



% With Perffuzz and Zest, we only need to implement generators 
% which are able to generate all possible states and all 
% possible events of the input services. 




% \subsection{Challenges and Tradeoffs}

% There are two extreme
% implementations of the performance fuzzer. 
% \leo{Do we need code example here?}
% One candidate implementation is to implement a universal 
% state generator that is able to generate all types of 
% data structures. For example, a direct memory mapping 
% generator maps the bit stream to the data structure 
% based on the memory layout of the data structure.
% However, such state generators may generate invalid states.
% In Figure~\ref{fig:host-store}, a direct memory mapping 
% generator may maps the same host to two different ids. 

% Another solution is to implement one fine-grain generator 
% for each data structure. The generator makes sure that all 
% states returned by the 
% generator are valid. For example, the host store generator 
% implements two map generators one for \texttt{hosts} and 
% one for \texttt{hostsByIp}.

% Figure~\ref{fig:host-store} presents the implementation 
% of host store which is the local state of the host service.
% Host store contains two maps \texttt{hosts} stores all 
% hosts indexed by ID and \texttt{hostsByIp} stores all 
% hosts indexed by IP. A naive memory mapping generator 
% is able to generate different instances of \texttt{hosts} and 
% \texttt{hostByIp}. However, the generator may also generate 
% invalid states where the host ID or host IP does not match host entities
% stored in map. On the other hand, if the developer decides to implement 
% generators for \texttt{hosts} and \texttt{hostsByIp}, they needs to 
% understand what are \texttt{HostId}, \texttt{Host}, and \texttt{IpAddress}, 
% and the relationship between different data structures.
% A naive generator which generates 
% random ID and host tuples may generate an invalid 
% host store. Therefore, implementing the state generator 
% is both time consuming and error-prone.


% Figure~\ref{fig:host-store}
% We use Figure~\ref{fig:host-store} as an example. 
% Figure~\ref{fig:host-store} presents the implementation 
% of host store which is part of the state of the SDN controller 
% storing the host information of the network.

% One way to implement generators is to implement generators 
% for each state and each event. Therefore, the more 
% state generators and event generators are implemented, 
% the more services can be analyzed. There are two 
% challenges to implement those generators. The first 
% challenge is that implementing 

% One way to implement performance fuzzer is to build state 
% generators and event generators for each service and use 
% Zest and Perffuzz to find a concrete state that may 
% have performance issue. However, states have internal 
% constraints that should be satisfied. The performance 
% fuzzer may report false positives if the state generator 
% generates invalid states. For example, 



\subsection{Our approach}

% \begin{algorithm}[t]
%   \input{figs/state-generator.tex}
%   \caption{State generator implemented with event generators.}
%   \label{fig:state-generator}
% \end{algorithm}

The key insight of our approach is that \emph{the number of 
types of events is much less than number of data structures 
in the SDN controller and the state changes in the SDN controller 
are driven by events}. 
 \vyas{i wonder if this is a top order insight that needs to be in sec 3? right now i wrote it as modular enables event in sec 3 but that may be incorrect these might be  two separate insights?} 
 

% The number of types of events in the SDN controller is much less than 
% the number of data structures implemented in the SDN controller.
Based on these observations, we propose event-driven state generators. 
{\systemname} implements a event generator which takes a bitstream 
as input and returns a sequence of events as output. For each 
sequence of events with length $N$, {\systemname} uses the first 
$N-1$ events to mutate the internal state of the input services 
and use the execution trace of the last event as the performance 
guidance for the underlying performance fuzzer. Thus, 
instead of implementing state generators for each data structure 
implemented in the SDN controller, {\systemname} only implements 
event generators. This approach assumes that given a sequence of 
valid events, {\systemname} will always produce a valid state.
% Given a sequence of valid events, \systemname
% will always generate a valid state.
% A event generator takes a bitstream as input and returns a sequence 
% of events as output. 
% A event generator $\fgenerator_{\feventtypelist_s}$ for service 
% $\fservice$ takes a bitstream as input and returns a sequence of 
% events as output.
% The event handler of service $\fservice$ is defined as 
% $\ffunction^\feventlist_\fservice::\langle\fstatetypelist_\fservice,
% \feventtype\rangle\rightarrow \langle\fstatetypelist_\fservice,\feventtype\rangle$.
% Figure~\ref{fig:state-generator} presents the proposed state generator 
% $\fgenerator_{\fstatetypelist_\fservice}$, 
% the state generator first initialize the state of the service to empty 
% state. It then uses event generator to generate a sequence of events. The 
% generator then iterates over all generated events and use event handler 
% to mutate the state $\fstate$. The event generator guarantees that 
% given a valid sequence of events, the event generator always generates a 
% valid state of the service.
% Therefore, instead of implementing both state generators 
% and event generators, {\systemname} only generates event generators 
% and rely on the generated events to generate different states of 
% the service.


\begin{algorithm}[t]
  \input{figs/fuzzing.tex}
  \caption{Fuzzing algorithm.}
  \label{fig:fuzzing}
\end{algorithm}

Figure~\ref{fig:fuzzing} shows the performance fuzzing algorithm
with event generators. The algorithm takes the analyzed services 
as well as its dependencies as input and returns 
a list of events that maximize the execution cost of the analyzed 
service.
% \leo{contribution:}
{\systemname} implements event generators which
converts a bitstream to a list of events.
$\finputlist$ stores a list of candidate bitstreams and 
is initialized to a random bitstream. Function $\mathrm{shouldContinue}$
is adopted from PerfFuzz~\cite{perffuzz} to decide when to stop fuzzing.
For each iteration, {\systemname} first resets the state of the 
analyzed service and the dependencies. Function $\mathrm{\mutate}$
is a function provided by the underlying fuzzer that mutates the current 
bitstream. Function $\fgenerator$ is the event generator that takes 
a bitstream as input and returns a sequence of events. 
{\systemname} uses all generated events except the last one to 
mutate the internal states of the input service and its dependencies.
{\systemname} then uses the last event in list $events$ and record 
the execution metrics. Function $\mathrm{shouldAddToInputList}$ is 
a method adopted from PerfFuzz~\cite{perffuzz} to decide if the new 
input should be stored in the input list.
If the execution cost of the new event sequence is larger then 
the stored one, {\systemname} updates the saved events and execution cost.
Finally, {\systemname} returns the event sequence that leads to the 
highest execution cost.
% $\mathrm{\fmutate}$ and $\mathrm{\fguidance}$ are two 
% core functions provided by PerfFuzz. $\mathrm{\fmutate}$
% function mutates a bitstream and returns a new bitstream 
% using its internal mutation algorithm. $\mathrm{\fguidance}$
% decides whether a bitstream should be added to the candidate 
% bitstreams $\finputlist$ based on the performance guidance. 
% $\fdata$ is the execution information collected 
% while executing the services $\fservicelist$.
% \vyas{im not sure what is the key idea or conceptual breakthrough. are you directly applying these tools? what is your contribution?}


==> files/hypothesis.tex <==
\section{Hypothesis}

There is a rich body of work on vulnerable SDN controllers 
with different techniques such as static analysis, dynamic 
analysis, and fuzzing. D2C2 detects vulnerabilities of SDN 
controllers which allows the attacker to increase the reachability 
in control plane by sending malicious packets~\cite{d2c2}.
However, D2C2 is not able to detect second-order 
data-to-control plan attacks because it does not have any knowledge 
about the performance impact of each network packet. Torpedo 
uses taint analysis to identify web APIs that allows an 
attacker to pollute database entires and call costly 
operations on those entires. It is not trivial to adapt 
Torpedo to SDN controllers because Torpedo relies on SQL queries
to identify which entry of the database can be polluted but 
such information is missing in SDN controllers.
Therefore, we believe that {\systemname} is both novel and 
unique.

Though the problem and the technique sounds promising, 
implementing such tool is still challenging because:

\begin{itemize}
  \item Dynamic analysis may report excessive data 
  structure and algorithm pairs, which cannot be modified 
  by data plan traffic. 
  \item In order to modify test input, {\systemname} needs 
  to understand the structure of the test cases and find 
  the location where test cases are generated.
  \item The most important and challenging task is to 
  implement an analysis tool which is able to tell not
  only if a data plane packet is able to modify a 
  data structure inside the SDN controller but also how 
  the data structure will be modified.
\end{itemize}

==> files/problem-statement.tex <==
\section{Problem Statement}


Software-defined networking (SDN) controller is a software that 
provides a centralized control of network control plane. 
In this work,
we are going to focus on second-order performance attacks \rp{vulnerabilities?}, 
which allows attackers to attack the SDN controller remotely~\cite{torpedo}. 

\vyas{it might be useful to define a threat model in terms of attacker goal and capabilities.} 
The attacker first injects malicious network events to manipulate 
states inside SDN controllers. They then send network 
events that cause costly operations on those states. 
Such second-order performance vulnerabilities are particularly severe because:
1) second-order attack traffics \rp{"traffics" is not a noun} can be sent in low frequency 
and mixed with normal traffics. Therefore, such malicious 
traffic are difficult for current intrusion detection systems; 
2) The SDN architecture \rp{controller?} is a 
single point failure of the controlled network \rp{architecture?} \rp{why is "single point of failure" important to your problem? does not look like you are studying reliability. "bottleneck" is probably more relevant}. Performance 
bugs in SDN controller will influence the performance of the 
entire network;
3) traditional analysis tool are not capable to 
detect such attacks because it involves state changes of the 
SDN controller.

\subsection{SDN Controller}

% \begin{figure}[t]
%   \input{figs/types.tex}
%   \caption{The types of the data structure.}
%   \label{fig:types}
% \end{figure}

% \begin{figure}[t]
%   \input{figs/predicate.tex}
%   \caption{Example predicates.}
%   \label{fig:predicate}
% \end{figure}

% It is also possible for a service to call a public function of another 
% service directly.
% A service $\fservice$ is an independent subsystem in the SDN controller. Each 
% service maintains a local state $\fstatelocal$ and all services maintain 
% a shared global state $\fstateglobal$. A state is a typed data structure.
% The input of the SDN controller is a sequence of OpenFlow messages, which 
% is the communication protocol between network switches and the SDN 
% controller~\cite{openflow}. There are two types of events in the SDN 
% controller. A packet event is used to communicate between services 
% and network switches. An internal event is used to communicate between 
% services. The SDN controller dispatches different 
% event to different services. The service will process 
% the OpenFlow message, update its local state and the global state, 
% and return a response OpenFlow message accordingly:
% $$
% \fservice :: \fevent \times \fstateglobal \times \fstate_\fservice 
% \rightarrow \fevent' \times \fstateglobal' \times \fstate_\fservice'
% $$

% Figure~\ref{fig:types} shows the types of states used in 
% the SDN controller. $T$ represents a set of primary types.
% $\mathrm{Int}$ is the integer type. The type 
% $\mathrm{List}\ T$ describes a mutable lists whose elements 
% have type $T$. The type $\mathrm{Set}\ T$ describes finite-length 
% set whose elements have type $T$. The type $\mathrm{Map}\ T$ 
% describes the map type whose field has an integer key and 
% a value with type $T$.
% The type
% $Record\ \{l_i: T_i^{i\in 1..n}\}$ describes the record 
% type with $n$ fields and each field has a label $l_i$ and 
% a type $T_i$.  
% Vertex, Edge, and Graph are three domain specific types based on 
% the primary type widely used in SDN controllers. 
% Vertex is an integer that represents a node in 
% a graph. Edge is a record containing two fields, source and destination,
% which represents a directed edge between two vertices. The graph type is 
% a record containing two fields, vertices and edges, that represents a 
% directed graph.

% Figure~\ref{fig:predicate} shows a list of 
% predicates on data structures. OneToOne predicate specifies that 
% each key of the map $\fdatastructure$ must points to distinct values.
% OneEdgeLeaving is a predicate on a graph whose
% every vertex has exactly one edge leaving it.
% ContainsKey predicate specifies that the map $\fdatastructure$ must
% contains the key $\finteger$. Contains predicate specifies that 
% the data structure $\fdatastructure$ must contain value $\fvalue$.
% A user may define other customized predicates using first order 
% logic.


\subsection{\systemname}

In this project, we build a system that takes the 
source code of a SDN controller $\fcontroller$ as input and 
generates a list of OpenFlow messages $\fofin$. We denote by $\fofin'$
\vyas{maybe some other notation like $M_{\prec i}$ maybe more intuitive}
the prefix containing the first $|\fofin| - 1$ messages and denote
by $\fofin^{-1}$ the last OpenFlow message. 
$\fofin'$ modifies the data
structure $\fdatastructurelist$ and $\fofin^{-1}$ 
triggers a costly service $\fservice$ which takes $\fdatastructure$ 
as input and will take more than $\fthresholdcpu$ to execute. \rp{Not sure where $D$ came from here. Might need to define how messages update data structures. Also, what is the difference between state and data structure?}

% \subsection{Existing Tools}

% \noindent\textbf{PerfFuzz\cite{perffuzz} and SlowFuzz\cite{slowfuzz}} 
% PerfFuzz and SlowFuzz are two performance analysis tools that 
% automatically generate input via feedback-directed mutational fuzzing.
% However, we cannot use those tools to analysis SDN controllers directly 
% because of lacking stateful input generation support.

% \noindent\textbf{AFLNet\cite{aflnet}} AFLNet is a stateful fuzzer 
% which takes a corpus of the recorded message between client and 
% server as input, and infers the state machine of the protocol.
% However, AFLNet utilize the request and response message to 
% determine the state of the server. It is not trivial to adopt 
% AFLNet to OpenFlow protocol directly because OpenFlow 
% protocols also include asynchronous messages.

% \noindent\textbf{Delta\cite{delta} and BEADS\cite{beads}} 
% Delta and BEADS are security audit tools design for SDN controllers. 
% Delta implements a stateful OpenFlow protocol fuzzer which is
% able to mutate and generate OpenFlow messages based on the current 
% state of the SDN controller. BEADS utilize mininet~\cite{mininet}
% and Open vSwitch~\cite{openvswitch} to generate stateful OpenFlow 
% messages and apply different mutation strategy to intercept 
% packets between switches and SDN controllers. However, both 
% tools requires a list of predefined attack strategies and does 
% not support performance attacks by default.

\subsection{Challenges}

In order to build a performance analysis tool \rp{Are you analyzing performance or trying to identify vulnerabilities? Analysis of performance is typically done by tools like profilers.} that is able to 
detect second-order performance vulnerabilities we need to solve the following 
challenges:
\begin{itemize}
  \item Because the SDN controller is a stateful system and accepts 
  infinite length of OpenFlow messages. It is not trivial to use
  traditional \vyas{who or what is traditional? } performance analysis tool to find input that cause 
  performance issues of the SDN controller.
  \item The ONOS SDN controller contains more than ten thousand 
  lines of Java code.
  \item The SDN controller stores all possible state \rp{Not sure what "all possible state" means. Won't the controller store only one state at any given time?} of the entire 
  network and the state space of the system is huge.
\end{itemize}

\vyas{feel like all three things are saying the  same things in different ways: 

maybe a different way to say it is the following: 
1. state space is huge. 
2. input-sequence space is huge. 
3. code space is huge.

and then maybe we can say how our insights tackle each problem?
}



\subsection{Insights}

Based on the design of the SDN controller and available tools, 
we have the following insights:

\begin{itemize}
  \item The SDN controller can be sliced into several subsystems and 
  analyzed individually.
  \item To analyze each subsystem, we need to find a concrete 
  sequence of events that causes the performance issue of the service.
  \item Each subsystem can be analyzed independently using an existing 
  data structure fuzzer.
  \item  
  % \item An OpenFlow message may have multiple consumers (services).
  % \item The service $\fservice$ has different processing time on different 
  % global state $\fstateglobal$, local state $\fstate_\fservice$, and 
  % OpenFlow message $\fof$.
  % \item A service may only read from and write to a subset of the global state 
  % $\fdatastructurelist$. For example, the host service of a SDN controller 
  % may never read from and write to the topology graph in the global state.
  % \item There is a set of constraints $\fconstraintlist$ on the global 
  % state $\fdatastructurelist$ which always hold.
\end{itemize}

\vyas{ideally we want the insights to tie back to the challenges eg the first bullet tackles the code problem. second idea tackles the state space problem.  third idea takcles packet problen etc etc} 


